Cosmology with Weak Lensing Surveys

Weak gravitational lensing is responsible for the shearing and magnification of the images of high-redshift sources due to the presence of intervening matter. The distortions are due to fluctuations in the gravitational potential, and are directly related to the distribution of matter and to the geometry and dynamics of the Universe. As a consequence, weak gravitational lensing offers unique possibilities for probing the Dark Matter and Dark Energy in the Universe. In this review, we summarise the theoretical and observational state of the subject, focussing on the statistical aspects of weak lensing, and consider the prospects for weak lensing surveys in the future. Weak gravitational lensing surveys are complementary to both galaxy surveys and cosmic microwave background (CMB) observations as they probe the unbiased non-linear matter power spectrum at modest redshifts. Most of the cosmological parameters are accurately estimated from CMB and large-scale galaxy surveys, so the focus of attention is shifting to understanding the nature of Dark Matter and Dark Energy. On the theoretical side, recent advances in the use of 3D information of the sources from photometric redshifts promise greater statistical power, and these are further enhanced by the use of statistics beyond two-point quantities such as the power spectrum. The use of 3D information also alleviates difficulties arising from physical effects such as the intrinsic alignment of galaxies, which can mimic weak lensing to some extent. (Abridged)

==> wl_P10.tex <==

\section{Gravitational lensing of supernovae}

Type Ia supernovae (SNeIa), which are believed to be the thermonuclear 
explosion of an accreting white dwarf, are standard candles with a small
intrinsic dispersion around their average luminosity. Moreover, this
dispersion can be further reduced to about $0.12$ mag using an empirical
relation between the peak magnitude and the width of the light curve
(Riess, Press \& Kirshner 1996). This makes SNeIa excellent tools for 
observational cosmology. In particular, by measuring their apparent magnitude
we can derive their distance from us and obtain the redshift-distance relation
up to $z\sim 1$ which provides useful constraints on cosmological parameters
(Goobar \& Perlmutter 1995). This method has supplied the main contribution to
the discovery of the present acceleration of the universe 
(Riess et al. 1998; Perlmutter et al. 1999) and it is the basis of future
proposals to probe the nature of dark energy through its equation of state
(e.g. the Supernova acceleration probe, Aldering et al. 2004).
On the other hand, SNeIa like all radiation sources are affected by 
gravitational lensing effects which can magnify or demagnify their observed
luminosity. This is a source of noise for studies which intend to measure
the redshift-distance relation but this effect may also be used by itself
to constrain cosmology in the same manner as gravitational lensing distortion
of distant galaxies. 

There are several important differences between SNeIa and galaxies as 
probes of gravitational lensing effects. Firstly, since SNeIa are point 
sources one uses the magnification (associated with the convergence $\kappa$) 
rather than the shear $\gamma$ which we focussed on in previous sections.
In particular, the magnification $\mu$ can be written as:
\beq
\mu = \frac{1}{(1-\kappa)^2-|\gamma|^2} \;\;\;\; \mbox{whence} \;\; \;\;
\mu\simeq 1+2\kappa \;\;\;\; \mbox{for} \;\;\;\; |\kappa| \ll 1, 
|\gamma|\ll 1 .
\label{mu}
\eeq 
Second, whereas weak gravitational lensing only modifies the observed
ellipticities of galaxies at $z_s=1$ by less than $10\%$, so that one needs
many galaxies to extract the signal, the magnification of a type Ia supernova
at $z_s=1$ by gravitational lensing is of the same order as the intrinsic
magnitude dispersion. Hence the signal-to-noise ratio is lager for SNeIa
but since we have many more observed galaxies than SNeIa accurate weak 
gravitational lensing effects have only been measured from galaxy 
ellipticities so far. 
Third, in order to derive the coherent shear on large scales one must
cross-correlate the observed ellipticities of many distant galaxies over
a window radius $\theta_s$ of the order of a few arcmin (since galaxies
are not exactly spherical). This leads to observables such as the aperture-mass
$\Map$ or the mean shear over scale $\theta_s$ which probe matter density
fluctuations over scales of the order of $\De\theta_s$. On the contrary,
the magnification of each SNeIa only probes the density fluctuations along
its line-of-sight, which corresponds to no smoothing ($\theta_s=0$). 
Then, by measuring the probability distribution of observed SNeIa magnitudes
(or its variance) rather than cross-correlating different SNeIa, one can 
probe the statistics of the convergence $\kappa$ with $\theta_s=0$. 
This means that the signal is dominated by scales where $\Delta^2(k)$ is 
maximum, which are set by the matter power-spectrum. For CDM power-spectra
this corresponds for sources at $z_s=1$ to wavenumbers $k \sim 10$ Mpc$^{-1}$
whereas smoothing galaxy ellipticities over $1$ arcmin mainly probes smaller
wavenumbers $k \sim 1$ Mpc$^{-1}$ (Valageas 2000). Thus, weak lensing
magnification of SNeIa allows us to probe density fluctuations on smaller
scales than with galaxy ellipticities. This also implies that non-Gaussianities
are more important for SNeIa gravitational lensing distortions.
On the other hand, this difference between the scales probed by galaxy
shear maps and SNeIa magnitude distortions means that both effects are
only weakly correlated so that weak-lensing shear maps obtained from 
surrounding galaxies are not very efficient to correct the SNeIa luminosities
(Dalal et al. 2003).

The rms magnification of SNeIa was computed by analytical means in 
Frieman (1997) who found that this would not significantly decrease the
accuracy of the distance-redshift relation at $z_s<0.5$ used to measure
the current acceleration of the universe but it could have a significant
effect at higher redshifts $z_s>1$, in agreement with the numerical
simulations performed in Wambsganss et al. (1997). In particular, although
future surveys covering more than a few square degrees will be unaffected,
pencil beams surveys ($<1$ deg$^2$) suffer significant contamination
(Cooray, Huterer \& Holz 2006).



\begin{figure}
\begin{tabular}{c}
{\epsfxsize=7cm\epsfysize=7cm\epsffile{PmuO03f.ps}}
{\epsfxsize=7.2cm\epsfysize=7.2cm\epsffile{wanggauss.eps}}
\end{tabular}
\caption{
{\it Left panel:}  the probability distribution $\cP(\mu)$ of the 
magnification within a $\Lambda$CDM universe for SNeIa at redshifts $z_s=0.5$
or $z_s=1$. From Valageas (2000a).
{\it Right panel:} the constraints on cosmological parameters obtained
from the dispersion of SNeIa magnitudes from a SNAP-like survey. The two sets
of contours correspond to analyzing the data assuming the true non-Gaussian
distribution (shaded) or a Gaussian distribution (unshaded).
From Dodelson \& Vallinotto (2006).
}
\label{fig:SNeIa}
\end{figure}



Turning to the use of SNeIa as a tool to detect gravitational lensing,
Metcalf (1999) computed analytically the rms magnification of SNeIa
to find that in a $\Lambda$CDM universe one needs at least $2400$ SNeIa
at $z_s=0.5$ (or $110$ SNeIa at $z_s=1$) to detect weak lensing from their
observed magnitudes. The PDF of the magnification $\cP(\mu)$ was computed
from a hierarchical model in Valageas (2000a) as well as its impact
on the measure of cosmological parameters through the distance-redshift 
relation. In particular, this study shows the strong non-Gaussianity
of the magnification with an extended high-$\mu$ tail which follows the
high-density tail of the underlying matter density field, as can be seen
from left panel of Fig.~\ref{fig:SNeIa}.
Then, the high-luminosity tail of observed SNeIa could be used to detect
weak-lensing since it should be significantly enhanced by gravitational
lensing. However, the number of observed SNeIa is still too small to
draw definite conclusions about a possible detection of weak lensing
effects by this method \cite{wang2005}.

On the other hand, since the amplitude of the gravitational lensing 
contribution to the dispersion of observed SNeIa magnitudes depends on
cosmological parameters it could be used to constrain cosmology
(Cooray, Holz \& Huterer 2006).
Thus, Dodelson \& Vallinotto (2006) found that $2000$ SNeIa in the redshift
range $0.5<z_s<1.7$ should be able to constrain up to $5\%$ the amplitude
$\sigma_8$ of the matter power-spectrum. However, they point out that
one needs to take into account the non-Gaussianity of the weak-lensing
magnification distribution in order to obtain correct estimates, as
seen in right panel of Fig.~\ref{fig:SNeIa}.

In order to eliminate the systematic errors associated with uncertainties
on the intrinsic SNeIa luminosity distribution and its possible dependence
on redshift, it is possible to cross-correlate SNeIa observed magnitudes
with foreground galaxies, as advocated in Metcalf (2001). Indeed, in the
absence of gravitational lensing this cross-correlation would vanish.
Using a halo model Metcalf (2001) found that a gravitational lensing signal
should be detected with $\sim 250$ SNeIa at $z_s=1$. This will be within the
reach of future experiments (e.g. the SNAP satellite should observe thousands
of SNeIa up to $z\sim 1.7$) but current surveys are too small to detect
a correlation between SNeIa magnitudes and galaxy overdensities
(Menard \& Dalal 2004).


